Neural Network Layers for Prediction of Positive Definite Elastic Stiffness Tensors

Machine learning models can be used to predict physical quantities like homogenized elasticity stiffness tensors, which must always be symmetric positive definite (SPD) based on conservation arguments. Two datasets of homogenized elasticity tensors of lattice materials are presented as examples, where it is desired to obtain models that map unit cell geometric and material parameters to their homogenized stiffness. Fitting a model to SPD data does not guarantee the model's predictions will remain SPD. Existing Cholsesky factorization and Eigendecomposition schemes are abstracted in this work as transformation layers which enforce the SPD condition. These layers can be included in many popular machine learning models to enforce SPD behavior. This work investigates the effects that different positivity functions have on the layers and how their inclusion affects model accuracy. Commonly used models are considered, including polynomials, radial basis functions, and neural networks. Ultimately it is shown that a single SPD layer improves the model's average prediction accuracy.

==> makefile <==
# $Id: makeFILE 193 2020-11-23 11:15:37Z rishi $

FILE=jekel_spd_nn_encorce_rev07_arxiv_ver
SHELL:=/bin/bash

all:
	lualatex -shell-escape -interaction=nonstopmode ${FILE}.tex; \
	bibtex ${FILE}.aux; \
	lualatex -shell-escape -interaction=nonstopmode ${FILE}.tex;

clean:
	rm -f ${FILE}.bbl ${FILE}.blg ${FILE}.spl ${FILE}.aux ${FILE}.log

